GTP-4o: Modality-prompted Heterogeneous Graph Learning for Omni-modal Biomedical Representation

Recent advances in learning multi-modal representation have witnessed the success in biomedical domains. While established techniques enable handling multi-modal information, the challenges are posed when extended to various clinical modalities and practical modalitymissing setting due to the inherent modality gaps. To tackle these, we propose an innovative Modality-prompted Heterogeneous Graph for Omnimodal Learning (GTP-4o), which embeds the numerous disparate clinical modalities into a unified representation, completes the deficient embedding of missing modality and reformulates the cross-modal learning with a graph-based aggregation. Specially, we establish a heterogeneous graph embedding to explicitly capture the diverse semantic properties on both the modality-specific features (nodes) and the cross-modal relations (edges). Then, we design a modality-prompted completion that enables completing the inadequate graph representation of missing modality through a graph prompting mechanism, which generates hallucination graphic topologies to steer the missing embedding towards the intact representation. Through the completed graph, we meticulously develop a knowledge-guided hierarchical cross-modal aggregation consisting of a global meta-path neighbouring to uncover the potential heterogeneous neighbors along the pathways driven by domain knowledge, and a local multi-relation aggregation module for the comprehensive cross-modal interaction across various heterogeneous relations. We assess the efficacy of our methodology on rigorous benchmarking experiments against prior state-of-the-arts. In a nutshell, GTP-4o presents an initial foray into the intriguing realm of embedding, relating and perceiving the heterogeneous patterns from various clinical modalities holistically via a graph theory. Project page: https://gtp-4-o.github.io/.

==> marco.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}

%%%%%%%%% PAPER TYPE  - PLEASE UPDATE FOR FINAL VERSION
\usepackage[review]{cvpr}      % To produce the REVIEW version
%\usepackage{cvpr}              % To produce the CAMERA-READY version
%\usepackage[pagenumbers]{cvpr} % To force page numbers, e.g. for an arXiv version

%%%%%%%%% PAPER ID  - PLEASE UPDATE
\def\cvprPaperID{3989} % *** Enter the CVPR Paper ID here
\def\confName{CVPR}
\def\confYear{2024}


% Include other packages here, before hyperref.
\usepackage[table]{xcolor}

\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{booktabs}

\usepackage{tikz}
\usepackage{comment}
\usepackage{amsmath,amssymb} % define this before the line numbering.}
\usepackage{bbm}
\usepackage{booktabs}
\usepackage[colorlinks, pagebackref]{hyperref}
\usepackage{graphicx}
\usepackage{bm}
\usepackage{multirow}

\usepackage{cases}

\usepackage{color}
\usepackage{ulem}

%\usepackage{algpseudocode}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{varwidth}
%\usepackage[ruled,vlined]{algorithm2e}

\usepackage{hyperref}
\usepackage{url}
\usepackage{times}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{multirow}
\usepackage{soul}
\usepackage{footnote}
\usepackage{tablefootnote}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{mathtools}


% \usepackage{varwidth}

% \usepackage{listings}
% \usepackage{xcolor}
% \usepackage{algorithm}
% \usepackage{algpseudocode}
% \usepackage{wrapfig}
% \usepackage{threeparttable}
% \usepackage{color, colortbl}
% \usepackage{multicol}
% \usepackage{multirow}

%\usepackage{subfig}

% It is strongly recommended to use hyperref, especially for the review version.
% hyperref with option pagebackref eases the reviewers' job.
% Please disable hyperref *only* if you encounter grave issues, e.g. with the
% file validation for the camera-ready version.
%
% If you comment hyperref and then uncomment it, you should delete
% ReviewTempalte.aux before re-running LaTeX.
% (Or just hit 'q' on the first LaTeX run, let it finish, and you
%  should be clear).
%\usepackage[pagebackref,breaklinks,colorlinks]{hyperref}

% Support for easy cross-referencing

\usepackage[capitalize]{cleveref}
\crefname{section}{Sec.}{Secs.}
\Crefname{section}{Section}{Sections}
\Crefname{table}{Table}{Tables}
\crefname{table}{Tab.}{Tabs.}

% \def\eg{\textit{e.g.}}
% \def\ie{\textit{i.e.}}
% \def\R#1{\,\ref{#1}}
% \def\RE#1{\,(\ref{#1})}

\definecolor{top1}{RGB}{255,179,179}
\definecolor{top2}{RGB}{255,217,179}
\definecolor{top3}{RGB}{255,255,179}



\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amstext}
\usepackage{amssymb}
\usepackage{booktabs}

\usepackage{tikz}
\usepackage{comment}
\usepackage{amsmath,amssymb} % define this before the line numbering.}
\usepackage{bbm}
\usepackage{booktabs}
\usepackage[colorlinks, pagebackref]{hyperref}
\usepackage{graphicx}
\usepackage{bm}
\usepackage{multirow}

\usepackage{cases}

\usepackage{color}
\usepackage{ulem}

%\usepackage{algpseudocode}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{varwidth}
%\usepackage[ruled,vlined]{algorithm2e}

\usepackage{hyperref}
\usepackage{url}
\usepackage{times}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{multirow}
\usepackage{soul}
\usepackage{footnote}
\usepackage{tablefootnote}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{mathtools}

\newcommand{\renyi}{{r\'enyi}}
\newcommand{\Renyi}{{R\'enyi}}
\newcommand{\fmm}[1]{{\textcolor[rgb]{1,0,0}{#1}}}
\newcommand{\rjc}[1]{{\textcolor[rgb]{0,0,0}{#1}}}
\usepackage[table]{xcolor}
% \definecolor{dino}{RGB}{249,231,227}

\usepackage{hyperref}
\usepackage{url}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage{pifont}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{algorithm}
\usepackage{mathtools}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{listings}
\usepackage{wrapfig}
\usepackage{subcaption}
\usepackage{xcolor,colortbl}

\newcommand{\cmark}{\color{green}\ding{51}}%
\newcommand{\xmark}{\color{red}\ding{55}}%
\newcommand{\yifan}[1]{{\color{blue}{[Yifan: #1]}}}


% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}


% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{hyperref}       % hyperlinks
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography
% \usepackage{xcolor}         % colors

% \usepackage{natbib}
% \usepackage{graphicx} 
% \usepackage{float} 
% \usepackage{amsmath}
% \usepackage{amsthm}
% \usepackage{subfig} 
% \usepackage{multirow,diagbox,enumitem}
% \usepackage{arydshln}
% \usepackage{graphicx}
% \usepackage{wrapfig}
% \usepackage{amssymb}
% \usepackage{makecell}

\newtheorem{example}{Example}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{definition}{Definition}
\newtheorem{proposition}{Proposition}

% \newcommand{\vpara}[1]{\vspace{0.05in}\noindent\textbf{#1 }}
% \newcommand{\vpait}[1]{\vspace{0.05in}\noindent\textit{#1 }}
% \newcommand{\noteblue}[1]{{\color{blue}#1}}

